HODN: Disentangling Human-Object Feature for HOI Detection

The task of Human-Object Interaction (HOI) detection is to detect humans and their interactions with surrounding objects, where transformer-based methods show dominant advances currently. However, these methods ignore the relationship among humans, objects, and interactions: 1) human features are more contributive than object ones to interaction prediction; 2) interactive information disturbs the detection of objects but helps human detection. In this paper, we propose a Human and Object Disentangling Network (HODN) to model the HOI relationships explicitly, where humans and objects are first detected by two disentangling decoders independently and then processed by an interaction decoder. Considering that human features are more contributive to interaction, we propose a Human-Guide Linking method to make sure the interaction decoder focuses on the human-centric regions with human features as the positional embeddings. To handle the opposite influences of interactions on humans and objects, we propose a Stop-Gradient Mechanism to stop interaction gradients from optimizing the object detection but to allow them to optimize the human detection. Our proposed method achieves competitive performance on both the V-COCO and the HICO-Det datasets. It can be combined with existing methods easily for state-of-the-art results.

==> Tables/combine.tex <==
\begin{table}[t]
    \centering
    \caption{Combination with existing works on both HICO-Det and V-COCO dataset.
        The performance we reported is Default Full on HICO-Det. And ${\mathrm{AP}}_{\mathrm{role}}^{\#1}$ and ${\mathrm{AP}}_{\mathrm{role}}^{\#2}$ are role mAP in scenario 1 and 2.
        In Backbone column, \textbf{R} represents ResNet.
    }
    
    \label{tab:combine}
    
    \resizebox{0.49\textwidth}{!}{
        \begin{tabular}{
            lllll
        }
        \toprule[1pt]
        \textbf{Method} & Backbone & 
        \textbf{HICO-Det} & 
        ${\mathbf{AP}}_{\mathrm{role}}^{\#1}$ &
        ${\mathbf{AP}}_{\mathrm{role}}^{\#2}$ \\ \midrule
        
        % DisTR~\cite{zhou2022human_distr} & R50 &
        % 31.75     & 66.2     \\
        % DisTR + HODN & R50 &
        % xx.xx ($\uparrow$ x.xx)     & xx.x ($\uparrow$ x.x)  \\
        % \hdashline[3pt/3pt]\rule{-3pt}{10pt}
        
        STIP~\cite{zhang2022exploring_stip} & R50 &
        32.22     & 66.0  &  70.7 \\
        STIP + HODN & R50 &
        xx.xx ($\uparrow$ x.xx)  & 66.6 ($\uparrow$ 0.6)  & 71.5 ($\uparrow$ 0.8)  \\
        \hdashline[3pt/3pt]\rule{-3pt}{10pt}
        
        GEN-VLKT~\cite{liao2022gen_genvlkt} & R50 &
        33.75     & 62.4  &  64.5 \\
        GEN-VLKT + HODN & R50 &
        xx.xx ($\uparrow$ x.xx)  & 65.2 ($\uparrow$ 2.8)  & 68.0 ($\uparrow$ 3.5)   \\
        
        \bottomrule[1pt]
        \end{tabular}
    }
    
\end{table}
    

==> sec_photo.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/smfang.jpeg}}]
{Shuman Fang}
received the B.E. degree from Beijing Institute of Technology, China, in 2020. She is currently pursuing the M.E. degree with the MAC Laboratory, Xiamen University. Her research interests include object detection and AI security. 
\end{IEEEbiography}
\vspace{11pt}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/zwlin.jpeg}}]
{Zhiwen Lin}
received the Master degree in computer engineering from Zhejiang University, Hangzhou, China, in 2019. He is currently a Researcher of Tencent Youtu Lab, Shanghai, China. His research interests include computer vision and deep learning.
\end{IEEEbiography}
\vspace{11pt}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/yke.jpeg}}]
{Ke Yan}
received the M.Sc. degree in computer science from Peking University, Beijing, China, in 2017. He is currently a Staff Researcher of Tencent Youtu Lab, Shanghai, China. His research interests include computer vision and deep learning.
\end{IEEEbiography}
\vspace{11pt}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/jli.jpeg}}]
{Jie Li}
received the B.E. degree from the Xiamen
University, China, in 2017. He is currently pursuing
his Ph.D. degree in the School of Informatics, Xia-
men University, China. His current research interests
include deep learning and computer vision.
\end{IEEEbiography}
\vspace{11pt}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/xmlin.jpeg}}]
{Xianming Lin}
is currently an Assistant Professor with Xiamen University, Xiamen, China. He received the Ph.D. degree in intelligent multimedia information processing from the School of Informatics, Xiamen University, Xiamen, China, in 2014. His current research interests include visual retrieval, computer vision, and machine learning.
\end{IEEEbiography}
\vspace{11pt}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/rrji.jpeg}}]
{Rongrong Ji}
is a Nanqiang Distinguished Professor at Xiamen University, the Deputy Director of the Office of Science and Technology at Xiamen University, and the Director of Media Analytics and Computing Lab. He was awarded as the National Science Foundation for Excellent Young Scholars (2014), the National Ten Thousand Plan for Young Top Talents (2017), and the National Science Foundation for Distinguished Young Scholars (2020). His research falls in the field of computer vision, multimedia analysis, and machine learning. He has published 50+ papers in ACM/IEEE Transactions, including TPAMI and IJCV, and 100+ full papers on top-tier conferences, such as CVPR and NeurIPS. His publications have got over 10K citations in Google Scholar. He was the recipient of the Best Paper Award of ACM Multimedia 2011. He has served as Area Chairs in top-tier conferences such as CVPR and ACM Multimedia.
\end{IEEEbiography}
\vspace{11pt}


\vfill
